When Should We Prefer Offline Reinforcement Learning Over Behavioral Cloning?

Offline reinforcement learning (RL) algorithms can acquire effective policies by utilizing previously collected experience, without any online interaction. It is widely understood that offline RL is able to extract good policies even from highly suboptimal data, a scenario where imitation learning finds suboptimal solutions that do not improve over the demonstrator that generated the dataset. However, another common use case for practitioners is to learn from data that resembles demonstrations. In this case, one can choose to apply offline RL, but can also use behavioral cloning (BC) algorithms, which mimic a subset of the dataset via supervised learning. Therefore, it seems natural to ask: when can an offline RL method outperform BC with an equal amount of expert data, even when BC is a natural choice? To answer this question, we characterize the properties of environments that allow offline RL methods to perform better than BC methods, even when only provided with expert data. Additionally, we show that policies trained on sufficiently noisy suboptimal data can attain better performance than even BC algorithms with expert data, especially on long-horizon problems. We validate our theoretical results via extensive experiments on both diagnostic and high-dimensional domains including robotic manipulation, maze navigation, and Atari games, with a variety of data distributions. We observe that, under specific but common conditions such as sparse rewards or noisy data sources, modern offline RL methods can significantly outperform BC.

==> todo.tex <==
Outline of the experiment section

1. RL w/ subopt data (expert + noisy expert; random data + expert data, unstructured random) > BC w/ expert data (Antmaze?)

2. Rl w/ expert data > BC w/ expert data (COG, Atari) --  critical points?  (Antmaze?)

3. [?] Sparse reward offline RL vs dense reward offline RL

4. Ablations of critical points: gridworlds, robomimic?; suboptimality and diversity ablation;  

Check structure with FA

======================================

Questions to resolve during revision:

1. Give names to the algorithms that we study, e.g. conservative RL, policy-constraint RL. I think one-step RL should be changed to have BC in the name to avoid potential confusion. Maybe BC + one-step policy-improvement?

2. I think the subsection titles in Section 4 are a bit misleading. In 4.2 (Expert Data), we compare BC to RL when they are both trained on expert data, which makes sense. However, in 4.3 (Noisy-Expert Data), we compare BC with expert data with RL with noisy expert data.

3. MissingMass still feels a bit awkward in that it it's only used to RL even though the BC bound would also contain it. 

4. How to reframe the critical points assumption. Also, make sure that it won't help BC.

5. Comments about Generalized BC section:

I think filtered BC is given an overly negative picture in this section. The advantage of these generalized BC methods should be for non-expert data, i.e. if the data is 80\% expert and 20\% noisy, then taking top-80\% would most likely decrease C^*. Overall, I think this section can perhaps be reframed to talk about methods that improve BC for non-expert data, but still don't improve enough to match RL.
